CoTAR: Chain-of-Thought Attribution Reasoning with Multi-level Granularity

State-of-the-art performance in QA tasks is currently achieved by systems employing Large Language Models (LLMs), however these models tend to hallucinate information in their responses. One approach focuses on enhancing the generation process by incorporating attribution from the given input to the output. However, the challenge of identifying appropriate attributions and verifying their accuracy against a source is a complex task that requires significant improvements in assessing such systems. We introduce an attribution-oriented Chain-of-Thought reasoning method to enhance the accuracy of attributions. This approach focuses the reasoning process on generating an attribution-centric output. Evaluations on two context-enhanced question-answering datasets using GPT-4 demonstrate improved accuracy and correctness of attributions. In addition, the combination of our method with finetuning enhances the response and attribution accuracy of two smaller LLMs, showing their potential to outperform GPT-4 in some cases.

==> archive/02-methods-backup.tex <==
\section{Method}
\label{sec:method}

\subsection{Citation Task Formulation}
\label{sec:cite_task_explain}

The general form of the tasks is as follows: given a question and a list of text passages, the goal is to answer correctly, while attributing aspects of the answer to the relevant passages; in other words the answer is expected to contain citations pointing to the passages. 

We can identify three forms of attribution: \textbf{passage, sentence and span}. These forms relate to the \textbf{answer structure}: whether the entire answer (passage) is attributed to one or more of the passages, each sentence can be attributed or individual spans in the answer are attributed to one or more of the passages. For an illustration, see \cref{fig:intro}.

In our setting, we are given a question $q$, a passage \peter{passage? the definition of attributable text needs to be defined and used in the same way throughput the paper} list $\{p_i\}_{i=1}^{K} = P$, and an expected answer list $\{a_i\}_{i=1}^{A}$.
\peter{whats the purpose of this passage? this is too obvious}Each passage $p_i$ could also be accompanied by a short gold answer, that is the essence of what the answer to the question should be from it. For example, if the passage is “Danny is 2 meters tall.” and the question is “How tall is Danny?”, the short gold answer will be “2 meters tall”. We denote the short gold answers as $G_k = \{G_{k}^{i}\}, k\in [1,K]$. 

\peter{this passage is too math-oriented and its very hard to understand the ideas of 3 levels of attribution.}
When generating answer $a$, with citations from the given passages $P$, we can identify three levels of citation.
Each citation $c=(c_p,c_s)$ is composed of the cited text $c_s$, and a passage index \daniel{it's not an index list, these are the actual passages, not their indices which is a subset of K not P} list $c_p \subseteq [1,K]$ that support $c_s$. Thus, the set of citations $C_t(a)$ for the current task $t$, contains all the citations of the given answer: $C_t(a) = \{c_m\}_{m}^{M_{a}^{t}}$, where $M_{a}^{t}$ is the number of citations for answer $a$ for task $t$. For clarity, we provide detailed examples for every citation level in Table \ref{tab:cite_level_example}.

\par \textbf{Passage Citation}: The entire answer is attributed to a subset of passages $P^{+} \subseteq [1,K]$, with no specific part being further attributed to any given passage. Hence, we have a \textbf{single} citation for our answer: $C_t(a) = \{(P^{+}, a)\}$.
\par \textbf{Sentence Citation}: Each sentence $s_j$ in the answer is attributed to a specific subset of passages $P_{j}^{+} \subseteq [1,K]$. Thus: $C_t(a) = \{(P_{j}^{+}, s_j)\}_{j=1}^{M_{a}^{t}}$.
\par \textbf{Span Citation}: The answer is composed of multiple cited text spans $C_t(a)$, and non cited text spans $NC_t(a)$. The cited spans can contain a single word, a phrase, or even multiple sentences. Each one \textit{must} be an exact excerpt from the a specific passage $p_{c_j}$, word for word, as proposed by \cite{Schuster2023SEMQASM}. For the scope of our work, even if the excerpt can be attributed to multiple passages, we attribute it to a single passage \peter{how? what are you doing?}. \peter{too much math .. }Thus: $C_t(a) = \{([p_{c_j}], sp_j)\}_{j=1}^{M_{a}^{t}}$, where $[]$ indicate a list, which in this case is a list with a single passage.



% PETER this passage has no relevancy, its obvious experimental stuff you mention.

% All COT types are applicable for all the tasks specified above.
% In the final evaluation, the COT prefix will not be considered in the evaluation metrics. 
% Instead, we only evaluate the final answer they decide to produce.

% Peter: this section is 1 experiment from our list of stuff in Exp setup section.
% \section{Citation-Level Finetuning}
% To further improve the model's ability to produce the corrected cited answers, we finetune our models based on each one of our datasets, and subsequently test them the their respective test sets. For this purpose, we perform finetuning for all three citation tasks, and for each of the three COT methods we have suggested above, including a method that includes no COT, which we denote as "Basic". The training hyperparameters can be found in Table \ref{tab:model_training_params}, and examples for the prompts used for training are provided in Table \ref{tab:prompt_span_level_example}. 



==> archive/03-preliminaries.tex <==
\section{Method}
\label{sec:methods-methods}

\subsection{Citation Task Formulation}

\daniel{Math is introduced here for the metrics definitions. Once we clean the metrics definitions we can come here and remove math that isn't needed.}

In our setting, we are given a question $q$, a passage \peter{passage? the definition of attributable text needs to be defined and used in the same way throughput the paper} list $\{p_i\}_{i=1}^{K} = P$, and an expected answer list $\{a_i\}_{i=1}^{A}$.
\peter{whats the purpose of this passage? this is too obvious}Each passage $p_i$ could also be accompanied by a short gold answer, that is the essence of what the answer to the question should be from it. For example, if the passage is “Danny is 2 meters tall.” and the question is “How tall is Danny?”, the short gold answer will be “2 meters tall”. We denote the short gold answers as $G_k = \{G_{k}^{i}\}, k\in [1,K]$. 

\peter{this passage is too math-oriented and its very hard to understand the ideas of 3 levels of attribution.}
When generating answer $a$, with citations from the given passages $P$, we can identify three levels of citation.
Each citation $c=(c_p,c_s)$ is composed of the cited text $c_s$, and a passage index \daniel{it's not an index list, these are the actual passages, not their indices which is a subset of K not P} list $c_p \subseteq [1,K]$ that support $c_s$. Thus, the set of citations $C_t(a)$ for the current task $t$, contains all the citations of the given answer: $C_t(a) = \{c_m\}_{m}^{M_{a}^{t}}$, where $M_{a}^{t}$ is the number of citations for answer $a$ for task $t$. For clarity, we provide detailed examples for every citation level in Table \ref{tab:cite_level_example}.

\par \textbf{Passage Citation}: The entire answer is attributed to a subset of passages $P^{+} \subseteq [1,K]$, with no specific part being further attributed to any given passage. Hence, we have a \textbf{single} citation for our answer: $C_t(a) = \{(P^{+}, a)\}$.
\par \textbf{Sentence Citation}: Each sentence $s_j$ in the answer is attributed to a specific subset of passages $P_{j}^{+} \subseteq [1,K]$. Thus: $C_t(a) = \{(P_{j}^{+}, s_j)\}_{j=1}^{M_{a}^{t}}$.
\par \textbf{Span Citation}: The answer is composed of multiple cited text spans $C_t(a)$, and non cited text spans $NC_t(a)$. The cited spans can contain a single word, a phrase, or even multiple sentences. Each one \textit{must} be an exact excerpt from the a specific passage $p_{c_j}$, word for word, as proposed by \cite{Schuster2023SEMQASM}. For the scope of our work, even if the excerpt can be attributed to multiple passages, we attribute it to a single passage \peter{how? what are you doing?}. \peter{too much math .. }Thus: $C_t(a) = \{([p_{c_j}], sp_j)\}_{j=1}^{M_{a}^{t}}$, where $[]$ indicate a list, which in this case is a list with a single passage.






==> archive/04-evaluation-metrics-backup.tex <==
\section{Evaluation Metrics}

In order to evaluate the answers produced by the various models, we specify multiple metrics, that address the following criteria:
\begin{itemize}
    \item \textbf{Answer Quality}: Similarity between the predicted answer and the gold answer.
    \item \textbf{Citation Quality}: Similarity between the cited text and the cited passage, and the citations present in the gold answer.
\end{itemize}

In the following sections, we describe the various metrics and how they relate to the main criteria we have named above.

\subsection{Answer Quality}

In order to measure answer quality, we employ several metrics; first we use the n-grams based methods ROUGE-L (RL) and F1 \cite{gao2023enabling, Schuster2023SEMQASM}. Additionally, we use the BERTScore metric \cite{bert-score}, which computes the cosine similarity between the vector representations of each token from the predicted answer, with the tokens from the target answer. 

\subsubsection{Hallucination Evaluation}

For hallucination evaluation in our predicted answers, we use the encoder model HEM\footnote{\url{https://huggingface.co/vectara/hallucination_evaluation_model}}, which was fine-tuned on NLI datasets, including TRUE \cite{honovich-etal-2022-true}, FEVER \cite{fever-2021-fact} and PWS \cite{paws2019naacl}, in order to predict whether two texts are factually consistent. We used it to compare the predicted answer with the expected answer.

\subsection{Citation Quality}

To measure the quality of the cited content, we propose specific metrics for each of the three forms of citation attribution---passage, sentence and span. One reason is that spans citations have to be correct at the word level, while sentence and passage attributions are not. 
\daniel{was: For all metrics, we denote a citation as $c = (c_s, c_p) \in C(a)$ as in \cref{sec:methods-methods}.}

\daniel{I would go passage, sentencne and then span here}

\subsubsection{Span Level Metrics}

The Span-Level metrics primarily focus on the direct word-for-word attribution of the span to the passage of origin. 

\paragraph{SEM F1:} Following SEMQA \cite{Schuster2023SEMQASM}, we measure the normalized token-F1 score between human annotated spans and predicted attribute spans, averaged over the number of passages. 

\daniel{was: For each passage we take all the spans predicted for this passage, and all the spans expected for this passage from the gold answers ${\hat{a}_i}$, and compute the token level F1 score between them.
The operation for taking all the spans of passage $p$ from answer $a$ is $\psi_{p}(a)$. 
We note that for our purposes, the comparison uses simple token-level-F1 scores, but we can compute more precise measurements. 
Since each question has multiple expected answers, we take the max score from them.
Formally, SEM F1 will thus be:
\begin{multline*}
\text{SEM\_F1}(a,{\hat{a}_i}) = \\ \frac{1}{K} \sum_{k\in [1,K]} \max_{\hat{a_i}}\, \text{F1}(\psi_{p}(a), \psi_{p}(\hat{a}_i))
\end{multline*}}

\paragraph{SEM REC:} Similarly to SEM F1, we measure token-recall score between short gold answers and predicted attribute spans. Higher scores represent higher coverage of correct answers with relevant attributions.

\daniel{was:
take all the spans predicted for this passage, and the \textit{short gold answer} for this passage, and compute the token level recall score between them
The comparison uses simple token-level-Recall scores, but we can compute more precise measurements. 
Since each passage could have multiple expected short answers, we take the max score from them.
Formally, SEM REC will thus be:
\begin{multline*}
\text{SEM\_REC}(a,G_{k}) = \\ \frac{1}{K} \sum_{k\in [1,K]} \max_{G_{k}^{i}\in G_{k}} \, \text{Rec}(\psi_{p}(a), G_{k}^{i})   
\end{multline*}}


\paragraph{Correct Citation Attribution (ATTR):}
We measure whether a predicted span is a direct span from the attributed passage by checking whether it is a valid sub-string, averaged over all predicted spans. 

\daniel{was: We check if a citation that the model provided is indeed a direct span from the specified passage. If it is, we count it as 1, else 0. The metric is the avertage across all the predicted citations.}

% \begin{equation}
% \text{CiteAttr}(a, P) = \frac{1}{|C(a)|} \sum_{c \in C(a)} I\{c_s \in p_{c_p}\}    
% \end{equation}

% \paragraph{Partial Citation Attribution:} Check if the model cited the span $c_p$ from at least one of the passages $p\in P$, even it not the from right one. This ensures that the span was at least not a hallucination:

% \begin{multline*}
% PartAttr(a, P) = \\ \frac{1}{|C(a)|} \sum_{c \in C(a)} I\{\exists p \in P: c_s \in p\}    
% \end{multline*}

% \paragraph{Noun Hallucination Ratio:} Check if every noun (nouns/proper nouns) produced by the model appears in the passages. This ensures that even though a span might not appear word-for-word in the passage, all the nouns specified by the model have not been hallucinated. We denote all the nouns of a string as $N(a)$:

% \begin{equation}
% Noun(a, P) = \frac{1}{|N(a)|} \sum_{no \in N(a)} I\{\exists p \in P: no \in p\}    
% \end{equation}

\subsubsection{Sentence and Passage Level Metrics}

\daniel{should be the same format as in the spans}

\paragraph{ALCE-R:} Following ALCE \cite{gao2023enabling}, we measure entailment between each cited sentence or paragraph and their corresponding attribution; we use an NLI model\footnote{\url{https://huggingface.co/google/t5_xxl_true_nli_mixture}} trained on the TRUE dataset \cite{honovich-etal-2022-true}. \daniel{I dont understand why is it recall}
-------This metric represents recall, as it examines the relevancy of the predicted citations. 

\daniel{was: For each citation $c\in C(a)$ at the sentence or passage level, check if $c_s$ is entailed from passages $c_p$. We define the $Ent(c_p, c_s)$ function as the logical entailment operation done by the TRUE model, with $c_p$ being the premise, and $c_s$ as the hypothesis.
\begin{multline*}
ALCERec(a) = \frac{1}{|C(a)|} \sum_{c \in C(a)} Ent(c_p, c_s)    
\end{multline*}}

\paragraph{ALCE-P} in order to measure precision, we predict whether a citation is \textbf{redundant} by using the NLI model to predict entailment of an answer from all citations excluding the citation in question \cite{gao2023enabling}. 

\daniel{was: In addition to the recall, \citet{gao2023enabling} also included ALCE Citation Precision. In the precision case, we consider each passage in the current citation $p\in c_p$. Let us remove it from the cited passages. If the text $c_s$ is not entailed from it, but \textbf{is} entailed from the all the others, then this is a \textbf{redundant passage}. We define the redundancy $R(p, c_p, c_s)$ as follows: 
\begin{multline*}
R(p, c_p, c_s) = \\ Ent(c_p / \{p\}, c_s) \wedge \neg Ent(\{p\}, c_s) 
\end{multline*}
Thus, the precision score for the current citation is the average amount of non-redundant passages:
\begin{equation}
Prec(c_p, c_s) = \frac{1}{|c_p|} \sum_{p\in c_p} I\{\neg R(p, c_p, c_s)\}
\end{equation}
For the final score, we average out across all the citations for the current answer:
\begin{multline*}
ALCEPrec(a) = \frac{1}{|C(a)|} \sum_{c \in C(a)} Prec(c_p, c_s)  
\end{multline*}}

\daniel{No need for a subsection, we are dealing with sentences and passages here; \subsection{Citation Recall and Precision}}

\daniel{Need a reorg or a better title, because everything before it was related to precision and recall}

\daniel{Are there metrics new and original? if so we need to say it}

\paragraph{DOC F1:} we calculate F1 score between the cited \textbf{passages} and the expected cited passages. 

\daniel{First, we define the set of all cited passages as:
\begin{equation}
CP(a) = \bigcup_{c\in C(a)} c_p   
\end{equation}
We note that for the sentence and passage level citation tasks, $CP(a)$ includes the passages attributed to the expected spans.
Then we compute the Doc Index F1 as the F1 score with the citations of the  expected answer $CP(\hat{a})$:
\begin{equation}
DocF1(a,{\hat{a}_i},P) = \max_{\hat{a_i}} F1(CP(a), CP(\hat{a}))
\end{equation}}

\paragraph{Disambig-F1:} following ASQA \cite{stelmakhASQAFactoidQuestions2022}, we use an extractive summary RoBERTa model \cite{Liu2019RoBERTaAR} to generate short summaries from the cited passages and compare them with the gold answers. \daniel{Did I get that right?}

\daniel{was: As described in \citet{Schuster2023SEMQASM}, this measurement involves using an extractive RoBERTa large QA model, \cite{Liu2019RoBERTaAR}, to operate on a series of clarifying queries and the produced long response. This process includes comparing each forecasted answer segment with the precise short-answer.}


